Quantum Modified Null Trajectories in Schwarzschild Spacetime

The photon vacuum polarization effect in curved spacetime leads to birefringence, i.e. the photon velocity becomes greater than (or less than) the speed of light depending on its polarization. We investigate this phenomenon in a Schwarzschild curved spacetime.

==> Acknowledgments.tex <==
\chapter{Acknowledgments}

There are many people to thank for their support and encouragement,
without whom this thesis would not have been possible. Firstly my
supervisors, Prof. Simon Hands and Prof. Graham Shore, for their
guidance, both academic and personal, throughout the course of my
postgraduate studies. Thanks also to my colleagues in the Swansea
particle theory group, Andrew Buxton, Steve Bidder and Iorwerth
Thomas. Also Aurora Trivini, with whom I have had many enlightening
discussions - physics related and otherwise. I also want to thank
all the friends I have made while living in Swansea, particularly
Robin Price, Antonio Di-Caprio, Gareth Coltman, Javier Silla, Jane
K\"{a}ehler, and Matthew Elwick.

I would like to thank both Swansea Physics Department and PPARC for
providing resources and funding for my research throughout this PhD.
\\
\\
Finally my family, to whom this thesis is dedicated, I cannot show
enough gratitude for the endless support and encouragement they have
given me.

